Divide&Classify: Fine-Grained Classification for City-Wide Visual Place Recognition

Visual Place recognition is commonly addressed as an image retrieval problem. However, retrieval methods are impractical to scale to large datasets, densely sampled from city-wide maps, since their dimension impact negatively on the inference time. Using approximate nearest neighbour search for retrieval helps to mitigate this issue, at the cost of a performance drop. In this paper we investigate whether we can effectively approach this task as a classification problem, thus bypassing the need for a similarity search. We find that existing classification methods for coarse, planet-wide localization are not suitable for the fine-grained and city-wide setting. This is largely due to how the dataset is split into classes, because these methods are designed to handle a sparse distribution of photos and as such do not consider the visual aliasing problem across neighbouring classes that naturally arises in dense scenarios. Thus, we propose a partitioning scheme that enables a fast and accurate inference, preserving a simple learning procedure, and a novel inference pipeline based on an ensemble of novel classifiers that uses the prototypes learned via an angular margin loss. Our method, Divide&Classify (D&C), enjoys the fast inference of classification solutions and an accuracy competitive with retrieval methods on the fine-grained, city-wide setting. Moreover, we show that D&C can be paired with existing retrieval pipelines to speed up computations by over 20 times while increasing their recall, leading to new state-of-the-art results.

==> figures/cp_viz.tex <==
\begin{figure}
    \begin{minipage}{.22\textwidth}
        \includegraphics[width=\textwidth]{images/viz/cp_0.jpg}
    \end{minipage}
    \begin{minipage}{.22\textwidth}
        \includegraphics[width=\textwidth]{images/viz/cp_0_small.jpg}
    \end{minipage}
\caption{\textbf{Size-based partitions applied on sf\_xl} Showing the first geoClass-set as in \textit{Cplanet}. The cells were generated using the s2sphere library fixed at the 18th level.   $|G|$.}
\label{fig:class-granularity}
\end{figure}


==> figures/roc.tex <==

\begin{figure}
    \includegraphics[width=\columnwidth]{images/roc_25_100.png}
    \caption{\textbf{ROC analysis} of Ours w/, w/o N,cosface vs competitors.}
    \label{fig:roc_analysis}
\end{figure}


==> tables/images_per_dataset.tex <==

\begin{table}
\begin{adjustbox}{width=\linewidth}
\centering
\begin{tabular}{lcccc}
\toprule
& SF-XL & C-Pitts30k & C-Pitts250k & C-Tokyo 24/7 \\
\hline
\# images & 41.2M & 30k & 254k & 76k \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Number of training images for each dataset.}}
\label{tab:images_per_dataset}
\end{table}


==> tables/supp_ablation_backbones.tex <==

\begin{table}
\centering
\begin{adjustbox}{width=0.75\linewidth}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Backbone} & 
\multicolumn{4}{c}{Great Circle Distance (GCD)} \\
\cline{2-5}
\multicolumn{1}{c}{}
& 25m & 50m & 100m & 500m \\
\hline
ResNet-50 \cite{He_2016_resnet}              & 52.0 & 54.7 & 55.6 & 59.0 \\
EfficientNet-B0 \cite{Tan_2019_efficientnet} & 49.2 & 52.8 & 53.5 & 57.8 \\
EfficientNet-B4 \cite{Tan_2019_efficientnet} & 54.3 & 57.1 & 57.6 & 61.5 \\
EfficientNet-B5 \cite{Tan_2019_efficientnet} & 56.9 & 60.0 & 60.1 & 63.3 \\
EfficientNet-B7 \cite{Tan_2019_efficientnet} & 62.1 & 64.9 & 65.4 & 67.6 \\
ViT \cite{Dosovitskiy_2021_vit}             & 48.9 & 51.5 & 52.2 & 57.1 \\
CCT \cite{Hassani_2021_cct}                 & 39.8 & 43.8 & 45.9 & 50.4 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Ablation on various backbones} on SF-XL.}
\label{tab:supp_ablation_backbones}
\end{table}


==> tables/supp_cplanet_distances.tex <==

\begin{table}
\begin{adjustbox}{width=\linewidth}
\centering
\begin{tabular}{l|cccc}
\toprule
 & SF-XL & C-Pitts30k & C-Pitts250k & C-Tokyo 24/7 \\
\hline
HGE-coarse & 23.41 & 20.27 & 21.09 & 42.00\\
HGE-medium & 14.37 & 13.16 & 12.26 & 24.86\\
HGE-fine   &  8.67 & 6.81 & 6.91 & 16.78\\
CPlaNet &  10.17 &  9.74 &   9.75 & 10.89 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Mean of distances between each image and the center of its class} \gb{TODO}}
\label{tab:supp_cplanet_distances}
\end{table}

